OpenGraphGym-MG: Using Reinforcement Learning to Solve Large Graph Optimization Problems on MultiGPU Systems

Large scale graph optimization problems arise in many fields. This paper presents an extensible, high performance framework (named OpenGraphGym-MG) that uses deep reinforcement learning and graph embedding to solve large graph optimization problems with multiple GPUs. The paper uses a common RL algorithm (deep Q-learning) and a representative graph embedding (structure2vec) to demonstrate the extensibility of the framework and, most importantly, to illustrate the novel optimization techniques, such as spatial parallelism, graph-level and node-level batched processing, distributed sparse graph storage, efficient parallel RL training and inference algorithms, repeated gradient descent iterations, and adaptive multiple-node selections. This study performs a comprehensive performance analysis on parallel efficiency and memory cost that proves the parallel RL training and inference algorithms are efficient and highly scalable on a number of GPUs. This study also conducts a range of large graph experiments, with both generated graphs (over 30 million edges) and real-world graphs, using a single compute node (with six GPUs) of the Summit supercomputer. Good scalability in both RL training and inference is achieved: as the number of GPUs increases from one to six, the time of a single step of RL training and a single step of RL inference on large graphs with more than 30 million edges, is reduced from 316.4s to 54.5s, and 23.8s to 3.4s, respectively. The research results on a single node lay out a solid foundation for the future work to address graph optimization problems with a large number of GPUs across multiple nodes in the Summit.

==> sections/background.tex <==
\section{Background}
\label{sec:background}

%basic knowledge for reader

% Section 2: Background: Graph Deep Reinforcement Learning\\ 0.5-1 
%     1) What is RL: keywords needed: Bellman Equation, reward r, and Return G, experience tuple, replay buffer. //RL: Arcade paper. RL introduction!
%     2) What is Graph DNN. Graph DNN. Supervised Graph Learning. GNN 
%       //Mainly about graph Training + Graph Embedding.
%       A Popular Field!
%     3) What is Graph RL: 1)+2). Unsupervised! Advantage: no label needed, ...

In this section, we first present a brief introduction to the reinforcement learning in Section \ref{subsec:rl_back}. Then, we discuss the graph embedding methods 
%which is the neural network to capture the information of graphs, 
in Section \ref{subsec:gnn_back}. Finally, we show how to combine RL and graph embedding to solve graph optimization problems in Section \ref{subsec:graphrl_back}.   
    
\subsection{Reinforcement Learning}
\label{subsec:rl_back}

% \begin{figure} [htb] %  figure placement: here, top, bottom, or page
%     \centering
% 	\includegraphics[width=0.45\textwidth]{figures/rl_workflow.pdf}
% 	\par \centering
% 	\caption{The workflow of Graph Reinforcement Learning}
% 	\label{fig:rl_worflow}
% \end{figure} 

%An \textit{Agent} learns ``correct'' behaviour by interacting with the \textit{Environment}. 
%In this section, we provide a brief introduction to reinforcement learning (RL). 
%Then, the training process of the RL agent will be explained. 
Reinforcement Learning (RL) is a process of trial-and-error interactions between the agent and the environment \cite{RLsurvey}. 
The goal of the RL agent is to train an optimal policy, which can lead to the maximal rewards in each episode. 

Before training, the \textit{RL agent} is responsible for initializing the \textit{policy model}. Policy model is the core of RL; it decides the actions based on the state. When the number of possible states is countable, a policy can be as simple as a look-up table \cite{qtable}.
%However, most policy functions in recent research are stochastic and able to tell which action is more possible to achieve better long-term reward. 
As to the computer vision and other applications, because of the large number of possible states, deep neural networks are more widely used as the policy model. %It has been proved that the deep neural network can help with many RL tasks \cite{rl_nature}.
%since the work of Mnih et al., where the Deep Neural Network model was firstly introduced \cite{rl_nature}.
%In this work, we use DRL.

Each \textit{episode} of the training process starts with the agent's exploring of a new problem instance. 
At every \textit{step} of a training episode, agent randomly or according to policy decides the action on the state. 
Then, the agent receives the \textit{reward signal} from the environment after applying that action.

The tuples of the state, reward and action are saved in the \textit{replay memory} denoted as $\{s^{}_{t}, a^{}_{t}, r^{}_{t+1}, s^{}_{t+1}\}$, where $s^{}_{t}$, $a^{}_{t}$, $r^{}_{t+1}$, $s^{}_{t+1}$ are the state at $t^{}_{th}$ step, action at $t^{}_{th}$ step, reward at $t+1^{}_{th}$ step, and state at $t+1^{}_{th}$ step.   
To train the policy model, the agent samples a batch of tuples from the replay memory.

Then, the agent applies the \textit{value function} to compute the ``labels" of the above tuples.
%After sampling, the agent evaluates an action and action using the value function.  
%to compute a target value for the policy model. 
The value function can take the intermediate reward and the future accumulative reward into consideration. \textit{Bellman equation} is often applied to simplify the value function. The Bellman equation for $t^{}_{th}$ step is as shown in Equation \ref{equa:bellman}, where $Q$ is the policy model.
\begin{equation}
\label{equa:bellman}
Q(s^{}_{t}, a^{}_{t}) = r^{}_{t} + \gamma \max\limits_{a^{}_{t+1}} Q(s^{}_{t+1}, a^{}_{t+1}) 
\end{equation}
% \added[id=Song]{It's not Bellman Equation. What is the LHS? Where is $a'$? Look at this link:}
% here I use s^{}_{t+1}, a^{}_{t+1} to replace s' and a', sorry for the confusing since it is another way of writing

% \url{https://medium.com/@curiousily/solving-an-mdp-with-q-learning-from-scratch-deep-reinforcement-learning-for-hackers-part-1-45d1d360c120}

Finally, each episode ends if a special \textit{termination state} has been reached. Then, the agent will start a new episode by exploring a new problem instance.   

% Bellman equation or other value functions is applied to compute the target Q value of the sampled tuples.   

% The major components of RL are as follows. 
% \begin{itemize}
%     \item{\textit{Agent:}} Agent is responsible for the learning of the way to map situations or states to actions. The goal of the agent is to maximize the sum of the reward signal at step.
%     \item{\textit{Environment:}} During the process of RL, environment perceives the action and provides the state to the agent.     
% 	\item{\textit{Policy Model:}} Policy is the core of the RL, it decides the action based on the states for the agent. When the number of possible states is accountable , policy can be as simple as a look-up table in some cases \cite{qtable}. However, most policy function in recent research are stochastic and used to tell agent which action is more possible to achieve better long-term reward. In the work of Mnih et. al, they create the deep reinforcement learning (DRL) and applied an Deep Neural Network as the policy model \cite{rl_nature}. In this work, we use the deep reinforcement learning (DRL).
% 	\item{\textit{Reward:}} Different from the \textit{supervised learning}, RL agent need to learn the correct value function by trying different actions. RL agent can receive a reward signal from the \textit{Environment} after trying an action every time.  
% 	\item{\textit{Value Function:}} Value function is used to evaluate an action and state in the longer term. The value function can not only take the intermediate reward, but also the accumulative reward in the future, into consideration. Bellman equation is often applied to simplify the value function. The value function for t-th step is as shown in equation \ref{equa:bellman}.
% 	\begin{equation}
%     \label{equa:bellman}
%     %\theta^{T}_{7} relu[\theta{}_{5} \sum\limits_{u\in V}^{} \mu{}_{u}, \theta{}_{6}\mu^{}_{v}]
%     r^{}_{t} + \gamma max Q(s^{}_{t+1}, a^{}_{t+1}) 
%     \end{equation}
%     $r^{}_{t}$ is the reward in t-th step. $s^{}_{t+1}$ and $a^{}_{t+1}$ are the state and action at (t+1)th step. Q is the policy function.  
% 	\item{\textit{Replay Memory:}} In DRL, replay memory is a data structure to store the tuples of experience $\{s^{}_{t}, a^{}_{t}, r^{}_{t+1}, s^{}_{t+1}\}$. At each step, agent will uniformly sample a batch of tuples from the replay buffer to train the policy model. 
% \end{itemize}



%In reinforcement learning, an agent and an environment interact with eachother  repeatedly  in every step.  For  eachstep,  the  agent  will  take  anaction,then the environment will provide the agent with arewardand the old and newstates. Eventually, the RL process will stop at a special “finished” state, whichis called theterminal state. The above sequence ofstepsuntilterminal stateis called anepisode.

% We considertasksin which the agent interacts with an environment
% througha sequence of observations, actions and rewards.The goal ofthe
% agent isto select actionsin a fashion that maximizes cumulative future
% reward. More formally,we use a deep convolutional neural network to
% approximate the optimal action-value function

\subsection{Graph Embedding}
\label{subsec:gnn_back}

The goal of the graph embedding is to represent the graph or node in a smaller dimension vector and efficiently 
preserve the graph structure and node information \cite{embed_survey}.

It is the foundation for many subsequent graph analytical problems such as the node classification, link prediction etc.   
%and has received a significant attention in last several decades. 
\added[id=Song]{Introduce more about Graph Embedding.}

\deleted[id=Song,comment={GNN sounds irrelevant here.}] {%\textit{GNN versus graph embedding:}
%Please note that the connections between the two emerging research areas graph embedding network and GNN are two folds.
%Inspired by the success of deep neural networks (DNN) in many research fields, researchers convert the DNN to graph neural network (GNN) for various graph applications \cite{gnn_survey, gnn_first, lecun_gnn}. 
%for the graph embedding techniques \cite{gnn_survey, gnn_first, lecun_gnn}. 
The differences between the GNN and graph embedding methods are two folds. 
On the one hand, GNN can support numerous graph applications, which includes the graph embedding task. In contrast, graph embedding network only targeting the representation of a graph or node. 
On the other hand, except the deep learning (GNN) based methods, researchers also use the matrix factorization, the graph kernel, the edge reconstruction, and the generative model based graph} %embedding methods \cite{embed_survey}. 


%GNNs are mostly supervised and label is needed to train the model. In contrast, the graph embedding network can be unsupervised. Please note that in this paper, we regard the unsupervised graph autoencoders as a deep learning based graph embedding network. 


\subsection{Deep Reinforcement Learning on Graphs}
\label{subsec:graphrl_back}

% \begin{figure} [htb] %  figure placement: here, top, bottom, or page
%     \centering
% 	\includegraphics[width=0.45\textwidth]{figures/grl_workflow.pdf}
% 	\par \centering
% 	\caption{The workflow of Reinforcement Learning to solve graph combinatorial optimization problem. Two steps are shown in the figure. }
% 	\label{fig:grl_worflow}
% \end{figure} 

Now, we are ready to introduce how to apply the RL algorithm to the graph optimization problems using the graph embedding network and the greedy solution building strategy. 
Greedy solution building strategy builds the solution of a problem instance by incrementally adding nodes to the graph. 
%\added[id=Song]{But the ``greedy solution building strategy'' has not been introduced so far.}

The formulation of the reward and the termination state need to be tuned based on the graph optimization problem. For the MVC problem, the reward equals the negative number of nodes to cover all edges at the end of each episode. When all the edges are covered, it reaches the termination state.  
During the training process, the RL agent first initializes a graph embedding network and a policy model. 
Then, the agent starts a new episode by creating a new environment using the randomly selected training graph. 
At each step of the training, the agent, either with its policy model or randomly, select one node and add it to the solution set. If the agent selects the node according to the policy model, two stages are \textit{Graph Embedding} and \textit{Candidate Nodes Evaluation}. At the first stage, we need to apply the graph embedding to all the vertices in the graph. Each candidate node will have a corresponding embedding vector. At the second stage, the RL policy model will take the embedding of all candidate nodes as the input and produce the Q scores. \textit{Graph agent} selects the node with the highest score and adds it to the solution set.
Similar to the common RL algorithm, the agent then updates the environment, pushes tuple to the replay buffer, and samples a batch of tuples from the replay buffer to train the graph embedding network and the policy model. Finally, the agent decides whether to start a new episode by checking the environment termination state. 

\added[id=Song]{The above whole subsection needs to be rewritten. It is so messy.}


%After selecting the node, the environment also update the graph environment. The agent also create a tuple and push it to the relay buffer. 
%Finally, at th






==> sections/backup.tex <==
%2D EM and Q model

\begin{algorithm}[b]
	\caption{Parallel Embedding Computation of \Call{EM}{$A^i$, $S^i$} on $\textbf{GPU}^{i}$}
	\label{alg:2d_parallel_em_model}
	\small{
		\begin{algorithmic}[1]
			
			\Input $A^{i}$: local subset of adjacency matrix of test graph (a sparse matrix) 
			\Statex \quad \ \ $S^i$: current partial MVC solution of the test graph  
			\State $K$: embedding dimension
            \State $L$: number of layers of embedding 
            \State $nGPUs$: number of GPUs
            \State $N$: number of nodes of the test graph 
            \State $N^i = N/nGPUs$: number of local subset of nodes of the test graph 
            
            \State $/*$ Parameters of the model: $*/$
			\State $\theta{}_{1}, \theta{}_{4} \in \mathbb{R}{}^{K \times 1}$; $\theta{}_{2}, \theta{}_{3} \in \mathbb{R}{}^{K \times K}$
			\State $/*$ Compute embedding for the local subset of nodes of the graph: $*/$
			
			\State $embed_1^i = \Call{DGEMM}{\theta{}_{1} , {(S^i)}^{T}}$    \Comment{ $\theta{}_{1} \in \mathbb{R}{}^{K \times 1}$, $S^i \in \mathbb{R}{}^{N^i \times 1}$}

    		\State $w^i$ = $\Call{ReLU}{\Call{SpMM}{\Call{reshape}{\theta{}_{4}, [K, N]}, {(A^{i})}^{T}}}$ 
    		\Statex \Comment{$A^i \in \mathbb{R}{}^{N^i \times N}$, dense-sparse matrix multiplication}

			\State $embed_2^i$ = $\Call{DGEMM}{\theta{}_{3}, w^i}$
        	\Comment{$\theta{}_{3} \in \mathbb{R}{}^{K \times K}$, $w^i \in \mathbb{R}{}^{K \times N^i}$ }

			\For{\texttt{layer $l = 1$ to $L$}}
			
			\State $embed_3^i = \Call{DGEMM}{\theta{}_{2}, embed^i}$  
    	    \Statex \Comment{$\theta{}_{2} \in \mathbb{R}{}^{K \times K}$, $embed^i \in \mathbb{R}{}^{K \times N^i}$} 
			\State $embed^i$ = $embed_1^i$ + $embed_2^i$ + $embed_3^i$ 
            \Statex \Comment{$embed_1^i$, $embed_2^i$, $embed_3^i$ $\in \mathbb{R}{}^{K \times N^i}$}
			\EndFor 
			
			\State return $embed^i$ \Comment{$embed^i \in \mathbb{R}{}^{K \times N^i}$}
            
		\end{algorithmic}
	}
\end{algorithm}

\begin{algorithm}[b]
	\caption{Parallel Q Value Computation of \Call{Q}{$embed^i$, $C^i$} on $\textbf{GPU}^{i}$}
	\label{alg:2d_parallel_q_model}
	\small{
		\begin{algorithmic}[1]
		 
			\Input $embed^{i} \in \mathbb{R}^{K \times N^i}$: computed embedding of local subset of nodes 
			\Statex \quad \ \ $C_{}^{i} \in \mathbb{R}^{N^i \times 1}$: local subset of candidate nodes
			\State $K$: embedding dimension
            \State $N^i = N/nGPUs$: number of local nodes of the test graph 

            \State $/*$ Parameters of the model: $*/$
			\State $\theta{}_{5}, \theta{}_{6} \in \mathbb{R}{}^{K \times K}$; $\theta{}_{7} \in \mathbb{R}{}^{2K \times 1} $
			
			% first we need to do sigma for the embeddings
% 			\State $/*$ Sum of the elements of ${embed}^{i}$, along axis 1 $*/$
			\State $/*$ $sum\_embed^i$ is the sum of the local subset of nodes' embeddings $*/$
			\State $sum\_embed^i$ =  $\Call{Sum}{embed^{i}, axis=1}$ 
            \Statex \Comment{ $embed^{i} \in \mathbb{R}{}^{K \times N^i}$, $sum\_embed^i \in \mathbb{R}{}^{K \times 1}$}
			
			\State $sum\_embed^{all}$ = $\Call{MPI-All-Reduce}{sum\_embed^i, op = sum}$ 

			\State $w_1^i = \Call{DGEMM}{\theta{}_{5}, sum\_embed^{all}}$
% 			\State $/*$ Please note that $sum\_embed^{all}$ is the all\_reduce sum of the ${sum\_embed}^{i}$, which is the sum of elements in ${embed}^{i}$ along axis 1 (Line 5) $*/$
            \Statex \Comment{ $\theta{}_{5} \in \mathbb{R}{}^{K \times K}$, $sum\_embed^{all} \in \mathbb{R}{}^{K \times 1}$}
			
            \State $/*$ create a sparse diagonal matrix using $\Call{sparse\_diag}{}$ $*/$
			\State $candidate\_embed^i$ = $\Call{SpMM}{embed^{i}, \Call{sparse\_diag}{C_{}^{i}}}$

			\Statex \Comment{$embed^{i} \in \mathbb{R}{}^{K \times N^i}$, $C_{}^{i} \in \mathbb{R}{}^{N^i \times 1}$, $\Call{sparse\_diag}{C_{}^{i}} \in \mathbb{R}{}^{N^i \times N^i}$}
			
			\State $w_2^i = \Call{DGEMM}{\theta{}_{6}, candidate\_embed^i}$
			\Statex \Comment{$\theta{}_{6} \in \mathbb{R}{}^{K \times K}$, $candidate\_embed^i \in \mathbb{R}{}^{K \times N^i}$}

			\State $w_3^i = \Call{ReLU}{\Call{Concat}{\Call{reshape}{w_1^i, [K, N^i]}, w_2^i}}$
			\Statex \Comment{$w_1^i \in \mathbb{R}{}^{K \times 1}$, $w_2^i \in \mathbb{R}{}^{K \times N^i}$}
			
			\State $scores^i = \Call{DGEMM}{{\theta{}_{7}}^{T}, w_3^i}$
			\Comment{$\theta{}_{7} \in \mathbb{R}{}^{2K \times 1}$, $w_3^i \in \mathbb{R}{}^{2K \times N^i}$}
			
			\State return $scores^i$ 	\Comment{$scores^i \in \mathbb{R}{}^{1 \times N^i}$}
			
		\end{algorithmic}
	}
\end{algorithm}



\begin{algorithm}[t]
	\caption{Parallel \Call{Tuples2SubGraphs}{tuples\_batch} on $\textbf{GPU}^{i}$ 
	\\/*needed by the parallel RL training Alg. \ref{alg:parallel_rl_training}*/
	I think we can skip this algorithm, and just describe its basic idea in the paper. It's too COO-specific.
	}
	\label{alg:paralleladj_update}
	\small{
		\begin{algorithmic}[1]
			%\State {\bf parallel\_testing}(Embed\_test, Q\_test, test\_G, P)
        	\Input tuples\_batch: a batch of sampled tuples from replay buffer
        	%Graph\_Dataset: a list pf training graphs
			%\Statex \quad \ \ tuples\_batch: sampled batch of tuples
			
			\State $list\_A^i$ = $\emptyset$: the list adjacency matrices
			\For{each $tuple$ in tuples\_batch}  

            \State $g$: the graph in $tuple$
			\State $A^{i}$: local subset of adjacency matrix for graph $g$ \Comment{in COO format}
			\State $S^{i}$: local partial solution in $tuple$

			\State $S = \Call{MPI-All-gather}{S^i}$
			\Comment{$S^i \in \mathbb{R}{}^{N^i \times 1}$}
			\State $row \xleftarrow{} \text{ row index array of matrix } A^{i}$
			\State $column \xleftarrow{} \text{ column index array of matrix } A^{i}$
			
			\For{\texttt{r in $nonzero(S)$}}
			\State $position$ = argwhere(column == r) //could be many positions?
			\State row.delete($position$); column.delete($position$)
			\EndFor
			
			\For{\texttt{r in $nonzero(S^i)$}}
			\State $position$ = argwhere(row == r)
			\State row.delete($position$); column.delete($position$)
			\EndFor
			\State $list\_A^i$.append(COO\_Matrix(row, column, values=1))
			\EndFor

			\State return $list\_A^i$
			
		\end{algorithmic}
	}
\end{algorithm}



\begin{algorithm}[tb]
	\caption{%Q-learning for the graph greedy algorithm training 
	RL for Graphs using Q-learning
	}
	\label{alg:greedy_rl}
	\small{
		\begin{algorithmic}[1]
			
			\Input Graph\_Dataset: a list of training graphs
			\Statex \quad \ \ $EM$: graph embedding model (to be trained)
			\Statex \quad \ \ $Q$: Q value model (to be trained)
			\State Replay\_Buffer = $\emptyset$: experience replay buffer 
			\State $B$: batch size
			\State MAX: number of training episodes 
			\State $T$: number of steps per episode
			\State $M$: number of delayed steps for receiving rewards
			
			\For{\texttt{episode $e = 1$ to $MAX$}}
			
			\State Tmp\_Replay\_Buffer = $\emptyset$: create a temporary replay buffer \par 
	        \hskip\algorithmicindent to store tuples with undecided target values

		    \State Randomly pick a graph ${g}^{}$ from \textit{Graph\_Dataset} 
		    \State $Env \xleftarrow{} \text{ Create a new environment using graph } {g}^{} $
		    %\State $adj = Graph$\_$list[g$\_$index]$
	    	\State $A$: adjacency matrix of graph ${g}^{}$
			
		    \State $S$ = $\emptyset$: current partial solution of graph ${g}^{}$
		    \State $C$: candidate nodes of graph ${g}^{}$

		    \For{each $step$ $t$} 
		    
		    \State
            $ v_{t}^{}=\left\{
            \begin{array}{@{}ll@{}}
            & \text{Randomly explore (select a node randomly), or} \\
            & \text{Model based exploit (using current model: $EM$, $Q$)}
            \end{array}\right.$
    
		    \State $S$ += $v_{t}^{}$; $C$ -= $v_{t}^{}$; Update $A$ based on $v_{t}^{}$
		    
		    % first push tuple to temporary replay buffer
		    \State Tmp\_Replay\_Buffer += (index of $g$; $S$; $v_t$;  $target\_value$=0)
		    
		    \If{$s \geq M$}
		    \State $reward$ = $Env.step(v_t)$, 
		    \State Compute the $target\_value$ using $reward$ of each 
	        \par \hskip\algorithmicindent \qquad \ 
	        tuple in Tmp\_Replay\_Buffer
		    \State Move updated tuples in Tmp\_Replay\_Buffer \par 
	        \hskip\algorithmicindent \qquad \ to Replay\_Buffer
			\EndIf
		    
		    \State tuples\_batch = sample(Replay\_Buffer, size=B)
		    
		    \State $/*$ Apply multiple iterations to train $EM$ and $Q$ $*/$
		    \State \Call{Train}{$Q$, $EM$, tuples\_batch} 
		    
		    \If{All edges are covered in graph ${g}$} break
		    \EndIf
			
			\EndFor
			\EndFor 
		
		\end{algorithmic}
	}
\end{algorithm}


\begin{table*}[tbp]
	\centering
	\caption{Definition of the RL algorithm components on Minimum Vertex Cover problem}
	\label{tbl:rl_elements}
	\small{
		\begin{tabular}{ | c | c | c | c | }
        \hline
        State & Subset of nodes selected as the partial solution \\
        \hline
        Action & Add a new node to the partial solution \\
        \hline
        Reward & Number of nodes used to cover edges at the end of the episode \\
        \hline
        Termination & All edges are covered \\
        \hline
        \end{tabular}
	    %}
	}
\end{table*}



\begin{algorithm}[bp]
	\caption{Embedding and policy model computation}
	\label{alg:model_imple}
	\small{
    	
		\begin{algorithmic}[1]
            \Input $A \in \mathbb{R}{}^{B \times N \times N}$: Adjacency matrices 
            \Statex \quad \ \ $S \in \mathbb{R}{}^{B \times 1 \times N}$: Partial solution nodes set
            \Statex \quad \ \ $C \in \mathbb{R}{}^{B \times N \times N}$: Candidate nodes set 
            \State $B$: batch size \Comment{equals 1 when applied to graph inference}
            \State $K$: embedding dimension
            \State $L$: number of layers of embedding 
            \State $N$: number of nodes in graphs 
            
            \State $/*$ Parameter variables of the model: $*/$
			\State $\theta{}_{1}, \theta{}_{4} \in \mathbb{R}{}^{K \times 1}$; $\theta{}_{2}, \theta{}_{3}, \theta{}_{5}, \theta{}_{6} \in \mathbb{R}{}^{K \times K}$; $\theta{}_{7} \in \mathbb{R}{}^{2K \times 1} $
			\State $/*$ The embedding of all nodes in graphs $*/$
			\State Initialize
			$embed \in \mathbb{R}{}^{B \times K \times N}$ to a zero tensor
			
			\State $/*$Submodel 1: Compute the embeddings for all nodes $*/$
			\State $embed_1$ = \Call{MatMul}{\Call{reshape}{$\theta{}_{1}$, $[B, K, 1]$}, S}
			\State $embed_3$ = \Call{MatMul}{\Call{reshape}{$\theta{}_{3}$, $[B, K, K]$},  \par 
	        \hskip\algorithmicindent \qquad \
	        \Call{ReLU}{\Call{MatMul}{\Call{reshape}{$\theta{}_{4}$, $[B, K, N]$}, A}}}
			
			\For{\texttt{layer $l = 1$ to $L$}}
			\State $embed_2$ = $\Call{MatMul}{\Call{reshape}{\theta{}_{2}, [B, K, K]}, embed}$ 
			\State $embed$ = $embed_1$ + $embed_2$ + $embed_3$

			\EndFor 
			
			\State $/*$Submodel 2: Compute Q values (scores) for candidate nodes$*/$
			\State $w_1$ = \Call{MatMul}{\Call{reshape}{$\theta{}_{5}$, $[B, K, K]$}, $\Call{Sum}{embed, axis=2}$}
		    \State $w_2$ = \Call{MatMul}{\Call{reshape}{$\theta{}_{6}$, $[B, K, K]$}, \Call{MatMul}{$embed$, $C$}}

			\State $w_3$ = \Call{ReLU}{\Call{Concat}{\Call{reshape}{$w_1$, $[B, K, N]$}, $w_2$}}; 
			%$w_3$ $\in \mathbb{R}{}^{B \times 2K \times N}$
			
			\State $scores$ = \Call{MatMul}{\Call{reshape}{$\theta^{T}_{7}$, $[B, 1, 2K]$}, $w_3$}
			\State return $scores$
			
		\end{algorithmic}
	}
\end{algorithm}



\subsubsection{\textbf{Graph Embedding and Q Value Model}} ~

%\subsection{Graph Representation: Graph Embedding and Q value Function}
\label{subsubsec:model_imple}



The agent's graph network model consists of two parts: 1) a graph embedding model
%\replaced[id=Song,comment={model or network? pick one.}]{model}{network}
, and 2) a Q value model. The two submodels are connected into one ``global'' model, that takes the original graph adjacency matrix as the input and outputs the scores for all solution candidate nodes.  
%\deleted[id=Song,comment={cannot be a solution.}]{solution}. 
The objective of connecting two models together is to tune and optimize both graph embedding and policy model for a specific type of graph optimization problems simultaneously.
We present the embedding and policy models in Alg. \ref{alg:model_imple}. 


The variables and parameters in Alg. \ref{alg:model_imple} are as follows. 
The mini-batch size \textit{B} is used in two different scenarios: 1) RL training and 2) graph inference.
As shown in Alg. \ref{alg:greedy_rl} Line 22, the agent samples a batch of tuples from the replay buffer to train the embedding and Q value models. 
In graph testing, we want to find optimal solutions for unseen graphs using the trained embedding and policy models. 
%\added[id=song]{Define what is Training, what is Testing here.}
In RL training, mini-batch size \textit{B} is equal to the number of experience tuples sampled from the replay buffer. The \textit{B} tuples, which correspond to \textit{B} graphs, are used to train the EM and Q model. 
%At the same time, \textit{B} is equal to 1 since there is only one action (i.e., one selected node) per experience tuple. 
In graph testing, \textit{B} is the number of unseen graphs. 
%and \textit{BN} is equal to the total number of candidate nodes per graph.
The parameters, $\theta{}_{1}$-$\theta{}_{7}$, will be ``learned'' by the agent's training process. 

%We also implement a matrix-tensor multiplication function, denoted by $\odot$, to multiply a 2D matrix with a 3D tensor, by performing a number of matrix multiplications in an embarrassingly parallel way.

\textbf{Graph Embedding Model} ~
%\label{subsubsubsec:embed_embed}


In Alg. \ref{alg:model_imple}, Lines 10-15 essentially compute the embedding vectors for a set of nodes using the following equation: %\ref{equa:emded} \cite{structure2vec}. 

\begin{equation}
\footnotesize{
\label{equa:emded}
\mu_v{}^{L} = relu(\theta{}_{1}x{}_{v} + \theta{}_{2} 
\sum\limits_{u\in N(v)}^{} \mu{}_{u}^{L-1} + \theta{}_{3} \sum\limits_{u\in N(v)}^{} relu(\theta{}_{4}(W(v, u)))),
}
\end{equation}

%\added[id=Song]{
where $\mu_v$ is the embedding vector of the nodes $v$ and $L$ is the index of the embedding layer. $N(v)$ represents the adjacent nodes of $v$. $W(v, u)$ is the weight of the edges between $v$ and $u$
%}
Note that Equation \ref{equa:emded} is only used to compute the embedding vector for a single node $v$, which is the same {\it structure2vec} function as introduced by Dai et al. \cite{structure2vec}. 
%Equation \ref{equa:emded} illustrates how to compute the embedding of node $v$ in the graph. 
%In Alg. \ref{alg:model_imple}

%\added[id=Song]{
However, to compute the embedding vectors for a set of nodes in a number of graphs simultaneously, we reformulate the problem into tensor computations, and then compute tensor operations for all the nodes and all the graphs in a batch. Here, we omit the mathematics steps
to convert a single-node embedding vector computation to a multi-graph and  multi-node embedding vector computation.
%} 
In the algorithm, Lines 10 and 11 are intended to compute $\theta{}_{1}x_{v}$
and $\theta{}_{3} \sum\limits_{u\in N(v)}^{} relu(\theta{}_{4}(W(v, u)))$ (in Equation \ref{equa:emded}) for all the nodes and all the graphs.
%that are included in the partial solution S, indicated in the equation. 
%As to the first term in the equation, $S{}_{v}$ is a binary number to indicate whether node $v$ is in the partial solution. 
%Also, in Line 2, $S$ is a 3D tensor including the solution information for all nodes, and $\theta{}_{1}$ is a 2D matrix. Hence, operator $\odot$ is invoked to multiply them.
Also, function {\it reshape} is used to convert an $E \times 1 $ matrix $\theta{}_{4}$ to a $B \times K \times N$ matrix by copying it $BN$ times.


In Lines 12-15, we show how to compute the graph embedding for a number of $L$ iterations, which
are implemented as $L$ layers.
%Please note that graph embedding computation includes $L$ layers of computations (as shown in Lines 3-5 in Alg. \ref{alg:model_imple}). Equation \ref{equa:emded} represents the computation of $L$-th layer.
In each iteration, we first multiply $\theta{}_{2}$ with $embed$, then add them to 
$embed_1$ and $embed_3$ to get the embedding for all the nodes for $B$ graphs.
%\sum\limits_{u\in N(v)}^{} \mu{}_{u}^{L-1}$ for all nodes 
%by multiply $\theta{}_{2}$ with $\mu$. 
%Then, we sum it up with the other two terms $\theta{}_{1}$' and $\theta{}_{3}$'. 
% The first and third term are constants. Thus, we compute the above two terms ($\theta{}_{1}$-term and $\theta{}_{3}$-term) before $L$ layers of embedding (Line 2 and 3 in Alg. \ref{alg:model_imple}). Then, we compute $L$ layers of embedding for all nodes in $B$ graphs (Lines 4-7).  
The final embedding result is a $B \times K \times N$ tensor, where each surface is a graph and each column of a surface is the embedding vector of a node.
%\todo{in the future, we need figures to show how it works.}



\textbf{Q Value Model} ~
%\label{subsubsubsec:embed_scores}

In Alg. \ref{alg:model_imple}, Lines 17-20 are used to compute the predicted Q values (or scores) for a set of nodes and a set of graphs. The model to compute the Q value for a single node is provided as follows.
%in Equation \ref{equa:scores}. 
\begin{equation}
\label{equa:scores}
Q_v=\theta^{T}_{7} relu[\theta{}_{5} \sum\limits_{u\in V}^{} \mu{}_{u}, \theta{}_{6}\mu^{}_{v}]
\end{equation}

Note that our Alg. \ref{alg:model_imple} can compute all the Q values for $BN$ nodes (i.e., $B$ graphs and each graph requests Q values of $N$ nodes) concurrently.
In Line 17, 
we first compute the term $\theta{}_{5} \sum\limits_{u\in V}^{} \mu{}_{u}$ (in Equation \ref{equa:scores}). 
$V$ is the set of all nodes in a graph. $\mu{}_{u}$ is the embedding vector of node $u$. As to the term $\sum\limits_{u\in V}^{} \mu{}_{u}$, we pool the embeddings of all nodes of a graph by summing them up. Then, we multiply the pooled embedding with $\theta{}_{5}$, 
and compute the term $\theta{}_{6}\mu^{}_{v}$.
Next, we concatenate the term $\theta{}_{5} \sum\limits_{u\in V}^{} \mu{}_{u}$ and $\theta{}_{6}\mu^{}_{v}$. 
The concatenated vector is relued in Line 19. Finally, we compute the Q values of the candidate nodes by multiply $\theta{}_{7}$ with the term $relu[\theta{}_{5} \sum\limits_{u\in V}^{} \mu{}_{u}, \theta{}_{6}\mu^{}_{v}]$. 
%shows the process of computing the score for node $v$. $\mu$ is the input of our Q function. Assume the $V$ is the collection of all nodes in a graph. In Alg. \ref{alg:model_imple} Line 9, we pooled the embeddings of all nodes. In Line 10, we compute the embeddings of all candidate nodes. Finally, as shown in Line 11 and 12, we concatenate the pooled embeddings and the candidate nodes embeddings in the first dimension. Finally, we compute the scores of candidate nodes using the cancatenated embeddings.



% \subsubsection{\textbf{Implementation in PyTorch}} ~
% \label{subsubsec:embed_imple}

% We use Pytorch \cite{pytorch} to implement the training and inference of the embedding and objective Q value models. 
% %The Pytorch code first defines the model (described in Alg. \ref{alg:model_imple}) as a dynamic computation graphs using Pytorch tensors. 
% It is relatively straightforward to follow Alg. \ref{alg:model_imple} and create variables for $\theta$'s and apply Pytorch operators to them.
% After the dynamic computation graph is created, we invoke the
% Pytorch training function 
% \textit{torch.optim.Adam(...).step()} 
% to launch the training procedure.




% \subsubsection{\textbf{Software Components}} ~
% \label{subsubsec:opengraphgym_components}
%\textit{Software Components:} 

% As shown in Fig. \ref{fig:framework}, 
% OpenGraphGym consists of three major software components:
% \begin{itemize}
% 	\item{\textit{Graph Learning Agent:}} Graph Learning Agent learns how to solve graph optimization problems through the reinforcement learning algorithm. The agent communicates with the Graph Network Model and the Graph Learning Environment by receiving the state, reward and sending the action information.  
% 	%from Graph Environment. 
% 	%\added[id=Song]{say sth like: by receiving the state info from env and using the DNN to make the best decision. }
% 	%The detailed introduction of this process is in Section \ref{subsec:rl_imple}.
% 	%It is the agent that is responsible for reinforcement learning for graph problems. It constantly receives input from three other components:
% 	%the $Neural$ $Network$ $Model$, the $Agent$ $Helper$ $Functions$, and the $Graph$ $Environment$. 
% 	%The $Neural$ $Network$ $Model$ provides DNN model output (e.g., Q values), the $Agent$ $Helper$ $Functions$ provides actions, and the $Graph$ $Environment$ provides states and rewards. On the other hand, the {\it Graph Learning Agent} also sends information to the three components constantly.
% 	\item{\textit{Graph Network Model:}} 
%     Graph Network Model defines the Graph Embedding Network and the Reinforcement Learning Policy Model. Embedding Network is responsible for generating the embedding vector for nodes. Policy Model can take the embedding vector as the input and output the Q values for candidate nodes. In Section \ref{subsec:model_imple}, we introduce an example of the Graph Network Model, which is structure2vec \cite{structure2vec}.  
% 	%It defines the graph embedding function and the RL agent's DNN model. 
%     %During RL training, the {\it Neural Network Model} takes a graph state as input and produces a {\it Q value}.
%     %The $Q$ value will be sent to the {\it Agent} for making decisions.
%     %In the current implementation of {\it OpenGraphGym}, we use the deep network Q-learning (DQN) method.
%     %Our next work will add the support of other RL methods such as A2C and A3C. 
%     \item{\textit{Graph Environment:}} 
%     Graph Environment receives the ``action" of how to modify the graph from the Graph Learning Agent. Then, it sends the new \textit{state} and checks whether the termination state has been reached after executing the ``action" over the graph.  
%     At the beginning of each episode, Graph Learning Environment creates a Graph Object. 
%     Each Graph Object has the adjacency matrix, the number of candidate nodes, edges, and other information of a graph.
%     By calling the function \textit{step}, Graph Learning Environment extract the reward and state from the Graph Object. In Alg. \ref{alg:greedy_rl}, we demonstrate the initialization and the function \textit{step} of the Graph Learning Environment.
%     %The $Graph$ $Environment$ is the interface between the $Graph$ and the $Graph$ $Learning$ $Agent$. $Action$, $reward$ and $state$ will be transferred through it.
% 	%\textcolor{black}{For example, when the $action$ is received from the $Graph$ $Learning$ $Agent$, the $Graph$ $Environment$ will call the function \textit{step} to send the $action$ to the component $Graph$. Then, it will receive the $state$ and the $reward$ from the component $Graph$. Finally, it will push the $state$ and the $reward$ to the $Graph$ $Learning$ $Agent$. %(need more details about what it is doing, and how it is done related to graphs....)}
% \end{itemize}


% \subsection{Software Libraries for the Implementation}
% \label{subsec:imple_opengraph_gym}

% Written in Python, OpenGraphGym framework use PyTorch \cite{pytorch} to define the Graph Network Model. PyTorch code defines the model 
% %(described in Alg. \ref{alg:model_imple}) 
% as a dynamic computation graph using PyTorch tensors. 
% %As shown in the section \ref{subsec:model_imple}, it is straightforward to follow Alg. \ref{alg:model_imple} and create variables for $\theta$'s and apply Pytorch operators to them.
% OpenGraphGym also use the graph library networkX \cite{networkx} in the Graph Learning Environment to generate different sizes of graphs and extract the basic information from a graph. 

% \subsection{Extensibility}
% \label{subsec:extensibility}

%OpenGraphGym framework is general since the testing of new graph embedding techniques, graph optimization problems and RL algorithms only requires changing some specific software components. 

% \subsubsection{\textbf{Extensibility}} ~
% \label{subsubsec:opengraphgym_extensibility}

% The OpenGraphGym framework can be extended to support different graph optimization problems, multiple graph embedding methods, and distinct RL algorithms.
% For example, to explore a new graph optimization problem, we just need to modify the environment \textit{constructor} and the \textit{step} function in the Graph Learning Environment. Now, we use Maximum Cut problem as an example to demonstrate how to extend \textit{OpenGraphGym}. 
% The goal of Maximum Cut (MAX) problem is to find a subset of nodes $S$ in an undirected graph such that the numnber of edges between $S$ and its complementary subset is as large as possible. The RL elements on MAX problem is as shown in Table \ref{tbl:rl_elements_max}.   
% As to the \textit{constructor}, we need to add a new local variable to record the number of edges between the solution set $S$ and its complementary set. For the \textit{step} function, the new function needs to calculate the corresponding reward and decide the termination state based on RL elements as shown in Table \ref{tbl:rl_elements_max}.

% Now, we use an example to show to extend {\it OpenGraphGym} to support other graph optimization problems.
% In the case of adding the Max Cut problem (MAX),
% we need to modify the $Graph$ component as shown in Fig.\ref{fig:architecture}. More specifically, two functions will be modified, which are: 1) the environment constructor (function \textit{\_\_init\_\_} in graph.py),
% and 2) the step function (function \textit{update\_state} in graph.py). 
% In the environment constructor, we need to add a new local variable to represent the cut set weight inside the environment initialization function. 
% In the step function, we then calculate the MAX-specific cut set weight to decide the termination state and the corresponding reward.
% Table \ref{tbl:rl_elements} shows the definitions of the reward and termination state for the MAX graph problem.

% \begin{table}[tbp]
% 	\centering
% 	\caption{Definition of the RL algorithm components on Maximum Cut problem}
% 	\label{tbl:rl_elements_max}
% 	\small{
% 		\begin{tabular}{ | c | c | c | c |}
%         \hline
%         State & Action & Reward & Termination  \\
%         \hline
%         Subset of & Add a & Number of nodes & Cannot find \\
%         nodes selected & new node & in the solution & a new \\
%         as the partial &  to the partial & at the end of & independent  \\
%         solution &  solution  & the episode & node \\
%         \hline
%         % Subset of nodes & Add a new & Number of nodes in & Cannot find a\\
%         % selected as the & node to the & the solution & new independent \\
%         % partial solution & partial solution & at the end of the episode & node \\
%         % & & & \\
%         % \hline
%         \end{tabular}
% 	    %}
% 	}
% \end{table}

% By adjusting the Graph Network Model, we can investigate new graph embedding methods. 
%\added[id=Song]{This is too simple. We need to introduce the programming API to let readers know how simple it is to extend it to support other graph problems, embedding methods, and other RL algorithms, if it is possible.}


%\subsection{limitation of the OpenGraphGym}
%\label{limit_opengraphgym}


% (Q1) A graph is too big to store on 1 GPU. //what did we do to solve it? 
% Q2) Our agent’s model is very complicated and need a careful design by using PyTorch. // e.g., we designed Sparse 3D Tensor, Zero Format Conversion, Dynamic generation of subgraphs, …. 
% Q3) The parallel inference and parallel training MultiGPU algorithms are totally new. 
% Q4) Even with our new parallel inference and parallel training algorithms, it is still time consuming. //So we design several optimization techniques.)

%OpenGraphGym only supports the testing and training on single GPU. The initial design of OpenGraphGym also does not scale well to handle large-scale graphs due to using a sequential inference process, dense matrix multiplication kernels, and unoptimized storage for graphs and replay buffers.

==> sections/framework.tex <==
\section{OpenGraphGym Framework and Solution Development }
\label{sec:framework}

%Section 3: Design of the software framework of OpenGraphGym\\
%    *Our contribution of the open framework design.
%    //Refer to ICCS paper. (don't copy anything).
%    +Multiple GPUs, PyTorch implementation, software libraries.
%    +Interface: open embedding, open graph problem/environment. why?

In this section, we provide an introduction to the OpenGraphGym framework. This open-source AI framework aims to facilitate the process of obtaining the solution for combinatorial graph optimization problem instances using deep reinforcement learning. 

\begin{figure} [t] %  figure placement: here, top, bottom, or page
    \centering
	\includegraphics[width=0.45\textwidth]{figures/framework_v3.pdf}
	\par \centering
	\caption{The OpenGraphGym Framework Architecture. Embedding Network belongs to the Graph Network Model.}
	\label{fig:framework}
\end{figure} 

\textit{Software Components:} As shown in Fig. \ref{fig:framework}, 
OpenGraphGym consists of three major software components:
\begin{itemize}
	\item{\textit{Graph Learning Agent:}} Graph Learning Agent learns how to solve graph optimization problems through the reinforcement learning algorithm. The agent communicates with the Graph Network Model and the Graph Learning Environment. 
	\added[id=Song]{say sth like: by receiving the state info from env and using the DNN to make the best decision. }
	The detailed introduction of this process is in Section \ref{subsec:rl_imple}. 
	%It is the agent that is responsible for reinforcement learning for graph problems. It constantly receives input from three other components:
	%the $Neural$ $Network$ $Model$, the $Agent$ $Helper$ $Functions$, and the $Graph$ $Environment$. 
	%The $Neural$ $Network$ $Model$ provides DNN model output (e.g., Q values), the $Agent$ $Helper$ $Functions$ provides actions, and the $Graph$ $Environment$ provides states and rewards. On the other hand, the {\it Graph Learning Agent} also sends information to the three components constantly.
	\item{\textit{Graph Network Model:}} 
    Graph Network Model defines the Graph Embedding Network and the Reinforcement Learning Policy Model. Embedding Network is responsible for generating the embedding vector for nodes. Policy Model can take the embedding vector as the input and output the Q values for candidate nodes. In Section \ref{subsec:model_imple}, we introduce an example of the Graph Network Model, which is structure2vec \cite{structure2vec}.  
	%It defines the graph embedding function and the RL agent's DNN model. 
    %During RL training, the {\it Neural Network Model} takes a graph state as input and produces a {\it Q value}.
    %The $Q$ value will be sent to the {\it Agent} for making decisions.
    %In the current implementation of {\it OpenGraphGym}, we use the deep network Q-learning (DQN) method.
    %Our next work will add the support of other RL methods such as A2C and A3C. 
    \item{\textit{Graph Environment:}} 
    Graph Environment receives the ``action" of how to modify the graph from the Graph Learning Agent. Then, it sends the new \textit{state} and checks whether the termination state has been reached after executing the ``action" over the graph.  
    At the beginning of each episode, Graph Learning Environment creates a Graph Object. 
    Each Graph Object has the adjacency matrix, the number of candidate nodes, edges, and other information of a graph.
    By calling the function \textit{step}, Graph Learning Environment extract the reward and state from the Graph Object. In Alg. \ref{alg:greedy_rl}, we demonstrate the initialization and the function \textit{step} of the Graph Learning Environment.
    %The $Graph$ $Environment$ is the interface between the $Graph$ and the $Graph$ $Learning$ $Agent$. $Action$, $reward$ and $state$ will be transferred through it.
	%\textcolor{black}{For example, when the $action$ is received from the $Graph$ $Learning$ $Agent$, the $Graph$ $Environment$ will call the function \textit{step} to send the $action$ to the component $Graph$. Then, it will receive the $state$ and the $reward$ from the component $Graph$. Finally, it will push the $state$ and the $reward$ to the $Graph$ $Learning$ $Agent$. %(need more details about what it is doing, and how it is done related to graphs....)}
\end{itemize}


% \subsection{Software Libraries for the Implementation}
% \label{subsec:imple_opengraph_gym}

% Written in Python, OpenGraphGym framework use PyTorch \cite{pytorch} to define the Graph Network Model. PyTorch code defines the model 
% %(described in Alg. \ref{alg:model_imple}) 
% as a dynamic computation graph using PyTorch tensors. 
% %As shown in the section \ref{subsec:model_imple}, it is straightforward to follow Alg. \ref{alg:model_imple} and create variables for $\theta$'s and apply Pytorch operators to them.
% OpenGraphGym also use the graph library networkX \cite{networkx} in the Graph Learning Environment to generate different sizes of graphs and extract the basic information from a graph. 

% \subsection{Extensibility}
% \label{subsec:extensibility}

%OpenGraphGym framework is general since the testing of new graph embedding techniques, graph optimization problems and RL algorithms only requires changing some specific software components. 
\textit{Extensibility:} The OpenGraphGym framework can be extended to support different graph optimization problems, multiple graph embedding methods, and distinct RL algorithms.
For example, to explore a new graph optimization problem, we just need to modify the environment constructor and the step function in the Graph Learning Environment. By adjusting the Graph Network Model, we can investigate new graph embedding methods. 
\added[id=Song]{This is too simple. We need to introduce the programming API to let readers know how simple it is to extend it to support other graph problems, embedding methods, and other RL algorithms, if it is possible.}


% \textcolor{black}{In this section, we demonstrate the extensibility of our framework from two perspectives: 1) how to support other graph optimization problems, and 2) how to add new graph embedding methods. %(write something in general first. Also, how to add a new embedding??)
% }

% Now, we use an example to show to extend {\it OpenGraphGym} to support other graph optimization problems.
% In the case of adding the Max Cut problem (MAX),
% we need to modify the $Graph$ component as shown in Fig.\ref{fig:architecture}. More specifically, two functions will be modified, which are: 1) the environment constructor (function \textit{\_\_init\_\_} in graph.py),
% and 2) the step function (function \textit{update\_state} in graph.py). 
% In the environment constructor, we need to add a new local variable to represent the cut set weight inside the environment initialization function. 
% In the step function, we then calculate the MAX-specific cut set weight to decide the termination state and the corresponding reward.
% Table \ref{tbl:rl_elements} shows the definitions of the reward and termination state for the MAX graph problem.

% \textcolor{black}{To demonstrate how to add the new graph embedding method, we will use an example of adding the node2vec embedding method. Node2vec is a graph embedding method aiming at preserving each node's neighborhood information \cite{node2vec}. We use the open-source node2vec library Node2Vec in our framework \cite{Node2VecLib}. Two functions needs to be modified in the $Graph$ component are 1) the environment constructor (function \textit{\_\_init\_\_} in graph.py), and 2) the step function (function \textit{update\_state} in graph.py). As to the environment constructor, we need to set up the node2vec model using the APIs provided by the Node2Vec library. As to the step function, we need to reset and update the node2vec model when the graph is modified. 
% }


% transition to next section: we use MVC as an example 



